VQ-T: RNN Transducers using Vector-Quantized Prediction Network States

Beam search, which is the dominant ASR decoding algorithm for end-to-end models, generates tree-structured hypotheses. However, recent studies have shown that decoding with hypothesis merging can achieve a more efficient search with comparable or better performance. But, the full context in recurrent networks is not compatible with hypothesis merging. We propose to use vector-quantized long short-term memory units (VQ-LSTM) in the prediction network of RNN transducers. By training the discrete representation jointly with the ASR network, hypotheses can be actively merged for lattice generation. Our experiments on the Switchboard corpus show that the proposed VQ RNN transducers improve ASR performance over transducers with regular prediction networks while also producing denser lattices with a very low oracle word error rate (WER) for the same beam size. Additional language model rescoring experiments also demonstrate the effectiveness of the proposed lattice generation scheme.

==> sections/0_Abstract.tex <==
abstract stuff

==> sections/1_Introduction.tex <==
introduction, related work

==> sections/2_CocktailSpeaker.tex <==
\section{Cocktail Speaker Model}
\subsection{Speaker Repr}
\subsection{Coktail Decoding}

==> sections/3_Experiments.tex <==
\section{Experiments}
\subsection{Evaluation}
\subsection{Baseline Approach}
\subsection{Results}
\subsection{Discussion}
